BioMiner: A Multi-modal System for Automated Mining of Protein-Ligand Bioactivity Data from Literature

Protein-ligand bioactivity data published in the literature are essential for drug discovery, yet manual curation struggles to keep pace with rapidly growing literature. Automated bioactivity extraction remains challenging because it requires not only interpreting biochemical semantics distributed across text, tables, and figures, but also reconstructing chemically exact ligand structures (e.g., Markush structures). To address this bottleneck, we introduce BioMiner, a multi-modal extraction framework that explicitly separates bioactivity semantic interpretation from ligand structure construction. Within BioMiner, bioactivity semantics are inferred through direct reasoning, while chemical structures are resolved via a chemical-structure-grounded visual semantic reasoning paradigm, in which multi-modal large language models operate on chemically grounded visual representations to infer inter-structure relationships, and exact molecular construction is delegated to domain chemistry tools. For rigorous evaluation and method development, we further establish BioVista, a comprehensive benchmark comprising 16,457 bioactivity entries curated from 500 publications. BioMiner validates its extraction ability and provides a quantitative baseline, achieving an F1 score of 0.32 for bioactivity triplets. BioMiner's practical utility is demonstrated via three applications: (1) extracting 82,262 data from 11,683 papers to build a pre-training database that improves downstream models performance by 3.9%; (2) enabling a human-in-the-loop workflow that doubles the number of high-quality NLRP3 bioactivity data, helping 38.6% improvement over 28 QSAR models and identification of 16 hit candidates with novel scaffolds; and (3) accelerating protein-ligand complex bioactivity annotation, achieving a 5.59-fold speed increase and 5.75% accuracy improvement over manual workflows in PoseBusters dataset.

==> tables/1_different_vllms.tex <==
\begin{table}[t]
 \centering
 \caption{Performance of \framework with different MLLMs on  \benchmark. This table focuses on presenting MLLMs-related results and comparing the performance of different MLLMs. In \framework, we choose Gemini-2.0-flash as our employed MLLM based on this table results.
 The best results are bolded, and the second best results are \underline{underlined.}}
 \label{tbl:overall_performance}
\begin{adjustbox}{width=1.0\textwidth}
\begin{threeparttable}
\begin{tabular}{cc|ccccccccccc}
\toprule
% \diagbox{Model}{Metric} 
Tasks & Metric & \textbf{Gemini-2.0-flash} & Gemini-2.0-pro & GPT-4o & GPT-4o-mini & Claude-3.7-sonnet & Claude-3.5-sonnet  & Grok-3 & Qwen-2.5 & \read{\MLLM(ours)} \\
\midrule
\multicolumn{6}{l}{\textit{Component-level evaluation for chemical structure extraction}} & & & & & & & &  \\
\midrule
\multirow{3}{*}{Full Structure Coreference} 
& Recall &  \textbf{0.786} & \underline{0.763} & 0.749 & 0.552 & 0.749 & 0.755 & 0.529 & 0.748 &  \\
& Precision & \textbf{0.783} & \underline{0.760} & 0.745 & 0.550 & 0.757 & 0.754 & 0.542 & 0.745 &  \\
& F1 & \textbf{0.784} & \underline{0.761} & 0.747 & 0.551 & 0.753 & 0.754 & 0.535 & 0.746 &  \\

\midrule
\multirow{3}{*}{Markush Enumerating w/ Coreference} 
& Recall & \textbf{0.579} & 0.386 & 0.430 & 0.039 & 0.465 & \underline{0.477} & 0.190 & 0.209 &  \\
& Precision & \textbf{0.545} & 0.377 & 0.426 & 0.041 & 0.475 & \underline{0.472} & 0.190 & 0.212 &  \\
& F1 & \textbf{0.561} & 0.381 & 0.428 & 0.040 & 0.470 & \underline{0.474} & 0.190 & 0.210 &  \\
\midrule
\multirow{3}{*}{Markush Enumerating w/o Coreference} 
& Recall & \textbf{0.628} & 0.425 & 0.500 & 0.050 & 0.503 & \underline{0.516} & 0.241 & 0.252 &  \\
& Precision & \textbf{0.594} & 0.448 & 0.495 & 0.058 & 0.514 & \underline{0.511} & 0.257 & 0.281 &  \\
& F1 & \textbf{0.611} & 0.436 & 0.497 & 0.054 & 0.508 & \underline{0.513} & 0.249 & 0.266 &  \\
\midrule

\multicolumn{6}{l}{\textit{Individual attributes evaluation for end-to-end extraction and annotation}} & & & & & & &   &  \\
\midrule

\multirow{3}{*}{Structure w/ Coreference} 
& Recall & \textbf{0.440} & 0.374 & 0.406 & 0.277 & \underline{0.436} & 0.434 & 0.275 & 0.373 &  \\
& Precision & 0.454 & 0.395 & 0.419 & 0.305 & \textbf{0.462} & \underline{0.459} & 0.326 & 0.403 &  \\
& F1 & \underline{0.447} & 0.384 & 0.412 & 0.290 & \textbf{0.449} & 0.446 & 0.298 & 0.387 &  \\

\midrule
\multirow{3}{*}{Bioactivity Measurement} 
& Recall & \textbf{0.594} & \underline{0.584} & 0.418 & 0.250 & 0.480 & 0.472 & 0.386 & 0.552 &  \\
& Precision & \textbf{0.486} & \underline{0.465} & 0.364 & 0.219 & 0.396 & 0.410 & 0.285 & 0.431 &  \\
& F1 & \textbf{0.535} & \underline{0.518} & 0.389 & 0.233 & 0.434 & 0.439 & 0.328 & 0.484 &  \\

\midrule
\multirow{3}{*}{Bioactivity Triplet} 
& Recall & \textbf{0.151} & \underline{0.141} & 0.107 & 0.055 & 0.130 & 0.130 & 0.067 & 0.122 &  \\
& Precision & \textbf{0.121} & 0.110 & 0.093 & 0.048 & 0.111 & \underline{0.115} & 0.050 & 0.092 &  \\
& F1 & \textbf{0.134} & \underline{0.124} & 0.100 & 0.051 & 0.120 & 0.122 & 0.057 & 0.105 &  \\

\midrule
\multirow{3}{*}{Bioactivity-Structure Annotation} 
& Top-1 & \underline{0.346} & 0.288 & 0.318 & 0.258 & 0.330 & \textbf{0.348} & 0.264 & 0.322 &  \\
& Top-3 & \textbf{0.544} & 0.482 & 0.530 & 0.454 & 0.518 & \underline{0.538} & 0.434 & 0.494 &  \\
& Top-10 & 0.686 & 0.634 & \underline{0.688} & 0.612 & 0.670 & \textbf{0.706} & 0.614 & 0.680 &  \\
\midrule
\multirow{2}{*}{1M Tokens Cost \$} 
& Input & \textbf{0.100} & 1.250 & 2.500 & \underline{0.150} & 3.300 & 3.300 & 0.830 & - &  \\
& Output & \textbf{0.400} & 5.000 & 10.000 & \underline{0.600} & 16.500 & 16.500 & 4.160 & - &  \\
% \midrule
% \multicolumn{2}{c|}{Average Rank} & \textbf{1.22} & 3.61 & 4.13 & 7.26 & 3.50 & \underline{3.24} & 6.70 & 5.07 \\
\bottomrule
\end{tabular}
\end{threeparttable}
\end{adjustbox}
\end{table}

